A Signal Injection Attack Against Zero Involvement Pairing and Authentication for the Internet of Things

Zero Involvement Pairing and Authentication (ZIPA) is a promising technique for autoprovisioning large networks of Internet-of-Things (IoT) devices. In this work, we present the first successful signal injection attack on a ZIPA system. Most existing ZIPA systems assume there is a negligible amount of influence from the unsecured outside space on the secured inside space. In reality, environmental signals do leak from adjacent unsecured spaces and influence the environment of the secured space. Our attack takes advantage of this fact to perform a signal injection attack on the popular Schurmann & Sigg algorithm. The keys generated by the adversary with a signal injection attack at 95 dBA is within the standard error of the legitimate device.

==> relatedwork.tex <==


\section{Related Work}

\todo[inline]{Shouldn't this really go earlier in the paper? I'd also use the LaTeX paragraph heading to make the two categories of related work stand out a bit. The discussion about AeroKey might help to answer my question earlier in the paper about what ZIPA devices are known to use the Sigg et al method.}
\label{sec:realted_work}
Our work focuses on the on stronger adversarial attacks on ZIPA systems.
Most ZIPA systems assume a weaker adversary for their threat model and thus perform weaker attacks on their systems.
Generally, threat models from prior work can be categorized in two ways: a passive adversary and a passive-active adversary.

\todo[inline]{The following paragraph should maybe go in the intro...}
\paragraph{Side Channel Attacks}
Cite Kevin Fu's work~\cite{fulaser,fulaser2,futemp,fudiskmic}.
Side channel attacks are coming out all the time.
New side channel attacks could be used to attack ZIPA systems.
Even if no injection attacks are known for a particular modality, it is possible that a new side channel attack could come out in the future.

For passive adversary threat model, the adversary watches and observes the context coming from the secured space from an unsecured space.
Typically, its assumed that an adversary only has access to the context observed from the unsecured space and does not try to actively try to manipulate the authentication process~\cite{Miettinen-CCS14,Saxena-S&P06,Mathur-Mobisys11}.

For the passive-active threat model, the adversary attempts to actively manipulate the authentication process through attacks such as replay attacks and machine learning attacks~\cite{aerokey,voltkey}.
A replay attack is where an adversary records the environmental context at an earlier time and replays it at a later time to masqurade as a legitimate device.
A machine learning attack is where a machine learning model is trained on environmental context collected at an earlier time to predict the environmental context later.
These threat models assume a stronger adversary, however this adversary is still unmotivated and weaker compared to our attack.

AeroKey~\cite{aerokey} is the only ZIPA system we know of that attempts a signal injection attack.
However, their signal injection attack was unsuccessful.
This could be due to a low injection signal intensity that cannot overwhelm the barriers of the secured space.
Also, the type of signal injected in AeroKey may not have been a good fit for the system's bit quantization algorithm.
% For example, measurements from ambient audio, received signal strength indicator (RSSI), visual channel and luminosity can be used to generate identical keys to establish secure communication channel~\cite{Miettinen-CCS14, Saxena-S&P06,Schurmann-TMC13, Mathur-Mobisys11}.
% Additionally,~\cite{Fomichev-UbiComp19} provides first large-scale public dataset of various devices in multiple environments (i.e., car and office) and re-evaluates various zero interaction pairing and authentication schemes. 

% In the wearable and mobile device domain, identical keys for pairing can be extracted from the legitimate user's electrocardiography (ECG) signal by extracting the time interval between two consecutive peaks from piezo or ECG sensors~\cite{Lin-IPSN19}. 
% To authenticate multiple mobile devices carried by the walking user,~\cite{Xu-IPSN16,Lester-Pervasive04} proposes key generation method from walking characteristics (gait) of the user based on their acceleration signal from different parts of their body.
% As an interactive pairing method,~\cite{Mayrhofer-CPC07} proposes device-to-device authentication by letting the user simultaneously shake two devices and use its movement patterns for key generation purposes. 

% Mechanical vibration context has proven to be useful for establishing a common secret only between colocated devices thanks to its proximity nature and the ubiquitous availability of accelerometers in various devices.
% Much like NFC and ultrasound~\cite{NFC,Ultrasound}, it can be used as an out-of-band communication channel to explicitly transmit and receive data using a vibration generator and an accelerometer~\cite{Kim-DAC15,  Roy-NSDI16,Saxena-PC11,Lee-ICCD18}, but it requires the devices to be in direct physical contact to transfer a secret generated by one device to another.
% Relevant research proposes to use vibration measured by multiple vehicles in the same lanes (a platoon of vehicles) to authenticate a newly joining vehicle for vehicle platooning purposes~\cite{Han-Hotmobile17}.
% Recently,~\cite{Groza-ACCESS19} addressed secure pairing of devices within multi-modal transport (i.e., train, tram, bike, and vehicle).
% Compared to this work, we specifically focus on the vehicular application with extensive experiments including adversarial attacks and multiple device locations under various road conditions and achieve consistently higher pairing success rates.


% \paragraph{Bit Distillation}
% Bit distillation algorithms take a bit stream as input and outputs a more random bit stream\cite{moonshine}.
% Common uses for bit distillation are applications where the platform is restricted to sampling randomness from a low-entropy source\cite{h2b}.
% The problem that bit distillation aims to solve is low randomness found in bit streams.
% We differ from bit distillation because we focus on composing time reliant sensor data to matching bit streams.


% \paragraph{Fuzzy Extractors}
% When sampling from an environmental noise source, there are cases where noise gathered from the same scene from two different perspectives does not match.
% Fuzzy extractors are algorithms that can account for different perspectives or slightly different readings from the environment to allow for stable use in cryptographic algorithms~\cite{juels1999fuzzy,juels2006fuzzy}.
% These algorithms are commonly used for biometric identification~\cite{maltoni2009handbook,sahai2005fuzzy}.
% %{\system} differs from the work in fuzzy extractors in that it generates a single matching key rather than allowing the key to differ.


